VINet: Visual and Inertial-based Terrain Classification and Adaptive Navigation over Unknown Terrain

We present a visual and inertial-based terrain classification network (VINet) for robotic navigation over different traversable surfaces. We use a novel navigation-based labeling scheme for terrain classification and generalization on unknown surfaces. Our proposed perception method and adaptive scheduling control framework can make predictions according to terrain navigation properties and lead to better performance on both terrain classification and navigation control on known and unknown surfaces. Our VINet can achieve 98.37% in terms of accuracy under supervised setting on known terrains and improve the accuracy by 8.51% on unknown terrains compared to previous methods. We deploy VINet on a mobile tracked robot for trajectory following and navigation on different terrains, and we demonstrate an improvement of 10.3% compared to a baseline controller in terms of RMSE.

==> vcl-shortcuts.tex <==
% This is roughly version 1.1 of vcl-shortcuts, circa Dec 2016.
% Put together by Vladlen Koltun

\usepackage{times}
\usepackage{epsfig}
% \usepackage{graphicx}
\usepackage{float}
\usepackage{wrapfig}
\usepackage{amsmath,amssymb}
%\usepackage{algorithm,algorithmicx,algpseudocode}
\usepackage{bm,xspace}
\usepackage{comment}
\usepackage{verbatim}
\usepackage{multirow}
\usepackage{balance}
\usepackage{url}
\usepackage{booktabs}
\usepackage{etoolbox,siunitx}
\usepackage{calc}
\usepackage{pifont,hologo}
\usepackage{xcolor}
%\usepackage[usenames, dvipsnames]{color}
%\usepackage{nicefrac}

\usepackage{multicol}
\usepackage{algorithm2e}
\usepackage{makecell}
\usepackage{arydshln}
\usepackage{multirow}
% \usepackage{ulem}
\usepackage{subcaption}

\usepackage{thmtools}
\usepackage{thm-restate}

%Set up nice tables using the tabular package
%Make \toprule and \bottomrule thicker than \midrule
\setlength\heavyrulewidth{0.10em}
\setlength\lightrulewidth{0.05em}
\setlength\cmidrulewidth{0.03em}
\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}

%Set up the siunitx package, particularly for using the S column type in tables
\usepackage[super]{nth}
\usepackage{nicefrac}
\sisetup{detect-weight=true,detect-inline-weight=math}
\sisetup{quotient-mode = fraction}
\sisetup{fraction-function = \nicefrac}
\robustify\bfseries

%Known issue: the following shortcuts override \gg, \ll\, and \tt, which are existing LaTeX commands. Use \ggreater and \llesser, defined below, instead of \gg and \ll. Use \texttt{} instead of \tt.
%Also \ss is taken and in some environments cannot be overridden. Use \sss for a bold `s' instead.
\def\aa{\mathbf{a}}
\def\bb{\mathbf{b}}
\def\cc{\mathbf{c}}
\def\dd{\mathbf{d}}
\def\ee{\mathbf{e}}
\def\ff{\mathbf{f}}
\def\gg{\mathbf{g}}
\def\hh{\mathbf{h}}
\def\ii{\mathbf{i}}
\def\jj{\mathbf{j}}
\def\kk{\mathbf{k}}
\def\ll{\mathbf{l}}
\def\mm{\mathbf{m}}
\def\nn{\mathbf{n}}
\def\oo{\mathbf{o}}
\def\pp{\mathbf{p}}
\def\qq{\mathbf{q}}
\def\rr{\mathbf{r}}
\def\sss{\mathbf{s}}
\def\tt{\mathbf{t}}
\def\uu{\mathbf{u}}
\def\vv{\mathbf{v}}
\def\ww{\mathbf{w}}
\def\xx{\mathbf{x}}
\def\yy{\mathbf{y}}
\def\zz{\mathbf{z}}

\def\AA{\mathbf{A}}
\def\BB{\mathbf{B}}
\def\CC{\mathbf{C}}
\def\DD{\mathbf{D}}
\def\EE{\mathbf{E}}
\def\FF{\mathbf{F}}
\def\GG{\mathbf{G}}
\def\HH{\mathbf{H}}
\def\II{\mathbf{I}}
\def\JJ{\mathbf{J}}
\def\KK{\mathbf{K}}
\def\LL{\mathbf{L}}
\def\MM{\mathbf{M}}
\def\NN{\mathbf{N}}
\def\OO{\mathbf{O}}
\def\PP{\mathbf{P}}
\def\QQ{\mathbf{Q}}
\def\RR{\mathbf{R}}
\def\SS{\mathbf{S}}
\def\TT{\mathbf{T}}
\def\UU{\mathbf{U}}
\def\VV{\mathbf{V}}
\def\WW{\mathbf{W}}
\def\XX{\mathbf{X}}
\def\YY{\mathbf{Y}}
\def\ZZ{\mathbf{Z}}

\def\aA{\mathcal{A}}
\def\bB{\mathcal{B}}
\def\cC{\mathcal{C}}
\def\dD{\mathcal{D}}
\def\eE{\mathcal{E}}
\def\fF{\mathcal{F}}
\def\gG{\mathcal{G}}
\def\hH{\mathcal{H}}
\def\iI{\mathcal{I}}
\def\jJ{\mathcal{J}}
\def\kK{\mathcal{K}}
\def\lL{\mathcal{L}}
\def\mM{\mathcal{M}}
\def\nN{\mathcal{N}}
\def\oO{\mathcal{O}}
\def\pP{\mathcal{P}}
\def\qQ{\mathcal{Q}}
\def\rR{\mathcal{R}}
\def\sS{\mathcal{S}}
\def\tT{\mathcal{T}}
\def\uU{\mathcal{U}}
\def\vV{\mathcal{V}}
\def\wW{\mathcal{W}}
\def\xX{\mathcal{X}}
\def\yY{\mathcal{Y}}
\def\zZ{\mathcal{Z}}

\def\Ae{\mathbb{A}}
\def\Be{\mathbb{B}}
\def\Ce{\mathbb{C}}
\def\Le{\mathbb{L}}
\def\Ne{\mathbb{N}}
\def\Pe{\mathbb{P}}
\def\Qe{\mathbb{Q}}
\def\Re{\mathbb{R}}
\def\Se{\mathbb{S}}
\def\Te{\mathbb{T}}
\def\Xe{\mathbb{X}}
\def\Ye{\mathbb{Y}}
\def\Ze{\mathbb{Z}}

\def\btheta{{\bm\theta}}
\def\bzeta{{\bm\zeta}}
\def\bmu{{\bm\mu}}
\def\bZero{\mathbf{0}}
\def\bOne{\mathbf{1}}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\minimize}{minimize}
\DeclareMathOperator*{\maximize}{minimize}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\trace}{tr}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\diam}{diam}

\def\eps{\varepsilon}
\def\vphi{\varphi}
\def\vsigma{\varsigma}

\def\trans{^{\top}}
\def\deg{^{\circ}}

\def\th{^{\textnormal{th}}}
\def\st{^{\textnormal{st}}}
\def\nd{^{\textnormal{nd}}}

%\ggreater and \llesser replace \gg and \ll, which have been overridden
\newcommand\ggreater{\mathbin{>\!\!\!>}}
\newcommand\llesser{\mathbin{<\!\!\!<}}

%Checkmark and cross symbols for tables
\newcommand{\YesV}{\ding{51}}%
\newcommand{\NoX}{\ding{55}}%

%Use @ instead of , in long numbers in math mode. For example, use $10@000$ rather than $10,000$.
\DeclareMathSymbol{@}{\mathord}{letters}{"3B}

\newcommand\paren[1]{\left(#1\right)}
\newcommand\abs[1]{\left\lvert#1\right\rvert}
\newcommand\norm[1]{\left\lVert#1\right\rVert}
\newcommand\tuple[1]{\left\langle#1\right\rangle}
\newcommand\inner[2]{\langle #1, #2 \rangle}

%Use \timess instead of \times in the main lines of equations, but not in superscripts or subscripts. Use the regular \times in superscripts or subscripts.
\newcommand\timess{\mathbin{\!\times\!}}

%Known issue: \nicebar is not nice in PNAS format, use \bar if submitting to PNAS.
\newcommand\nicebar[1]{\mkern 4mu\overline{\mkern-4mu#1}}

%Replace ``\yourname" and ``Name" with your name
\newcommand\yourname[1]{\textcolor{blue}{Name says: #1}}
\newcommand\vladlen[1]{\textcolor{blue}{Vladlen says: #1}}

%Paragraph heading with customizable vertical spacing. Modify the length inside \vspace to expand or contract the vertical offset preceding a new paragraph heading.
\newcommand\mypara[1]{\vspace{1mm}\noindent\textbf{#1}}

%Orient text vertically. Useful for tables and figures.
\def\rot#1{\rotatebox{90}{#1}}

%I use the self-indulgent \LaTeX operator mostly to illustrate an issue and a useful trick. The issue is that LaTeX operators eat the space that follows them, so if they occur in the middle of a sentence they eliminate the space separating the following word. But you can't just insert a space will-nilly (e.g., \LaTeX\ or \LaTeX~) because if the operator is followed by a punctuation mark then there shouldn't be a space. One solution is to write \LaTeX{}, which does the right thing but is easy to forget. The alternative, demonstrated here, is to define an operator with a name that ends with the forward slash. This also does the right thing and looks sufficiently distinctive to be memorable.
\def\latex/{\LaTeX}
\def\bibtex/{\hologo{BibTeX}}

%Miscellaneous \latex/ tips:
% To create an invisible character, use the \phantom command or its relatives: http://tex.stackexchange.com/questions/4519/how-do-i-create-an-invisible-character

